Understanding and Evaluating Developer Behaviour in Programming Tasks

To evaluate how developers perform differently in solving programming tasks, i.e., which actions and behaviours are more beneficial to them than others and if there are any specific strategies and behaviours that may indicate good versus poor understanding of the task and program given to them, we used the MIMESIS plug-in to record developers' interactions with the IDE. In a series of three studies we investigated the specific behaviour of developers solving a specific programming task. We focused on which source code files they visited, how they related pieces of code and knowledge to others and when and how successful they performed code edits. To cope with the variety of behaviours due to interpersonal differences such as different level of knowledge, development style or problem solving stratiegies, we used an abstraction of the observed behaviour, which enables for a better comparison between different individual attributes such as skill, speed and used stratiegies and also facilitates later automatic evaluation of behaviours, i.e. by using a software to react to.

==> mimesis.tex <==
\section{The \mimesis Tool}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\textwidth]
%    {img/visDetailRange2} % \\[\medskipamount]
% %   \includegraphics[width=.75\textwidth]
% %   {img/legend} \\[\smallskipamount]
%   \caption{Interactive visualisation of a development session recorded with the 
% \mimesis plug-in.} 
%   \textit{Lines in the visualisation indicate navigation between 
% lines and files, areas indicate the range of lines visible on the 
% screen, symbols display invididual events. Specific events can be selected 
% either from the graph-like visualisation or from a comprehensive sequential 
% list. Both selection methods offer additional detailed information about the 
% corresponding event, either using a tooltip in the visualisation or a drop down 
% list of attributes in the event list.}
%   \label{fig:visualisationOverview}
% \end{figure*}

While a number of specific aspects of the process of program comprehension were 
identified by related works, those works describe particular fragments of 
program comprehension, investigate specific contexts using indirect 
measurements like video recording~\citep{piorkowski2013whats, 
baltes2015navigate}, think aloud methods~\citep{roehm2012professional, 
grigoreanu2012strategies, 
lawrance2013programmers} or surveys~\citep{sadowski2015developers}, or provide 
models~\citep{sillito2008asking} to describe program comprehension that seem too 
abstract to be observed in actual developer behaviour. 
Complementing existing related work on the topic, we intended to provide a 
holistic approach to investigate developer behaviour, i.e., by recording all 
interactions performed while solving development tasks, our approach is generic 
enough to allow investigation of arbitrary tasks and contexts (e.g., modifying 
existing code, writing new code, using documentation), yet, by capturing 
fine grained interaction and navigation events, it also is specific enough to 
provide detailed insights into developer behaviour "at runtime".
% To proof this concept, we performed a study in which we intended to observe 
% some of the aspects reported in related work in the data of actual interactions
% recorded by our tool, especially such as the different navigation behaviours so 
% far only observed indirectly or just assumed in other 
% works~\citep{roehm2012professional, piorkowski2013whats, minelli2014visualizing, 
% minelli2015know}.
% In our research, we were interested to record interactions of developers working 
% on programming tasks. 
% Complementary to other approaches which used video 
% recordings~\citep{piorkowski2013whats, baltes2015navigate} or think aloud 
% methods~\citep{roehm2012professional, grigoreanu2012strategies, 
% lawrance2013programmers} 
%To achieve this, we chose to capture those interactions using a plug-in for 
We chose to capture those interactions using a plug-in for the 
\textsc{Eclipse} IDE, 
% We did this because we want to provide an efficient method, i.e., suitable 
% for automatic (pre-)processing, which is yet able to consistently collect 
% interaction data, as we focus on the comparison between developers and 
% between development tasks rather than on individual characteristics of 
% developers or tasks.
% This approach enables 
enabling us to perform scalable observations suitable for 
automatic (pre-)processing without the need of an observer present at the 
recording, which also enables \textit{remote participation}, i.e., providing 
subjects with a downloadable bundle containing a preconfigured IDE with the 
plugin and the task to be solved.
% link where a bundle containing a preconfigured IDE with the 
% plugin and the task to be solved can be downloaded. 
% Alternatively, and expecially t
To avoid the need to download anything to a participant's computer, this 
configuration bundle % of the IDE and an experimental task can be provided in a 
can also be provided in a way that enables subjects to participate by just using 
their browser to connect to a desktop environment precofigured for the 
experiment.
This allows subjects to participate at home or from their usual work 
environments and remotely contribute the recorded data.

% \pagebreak
Beyond the recording of interaction data, our tool---which we dubbed 
\mimesis---also allows for the interactive visualisation of such 
recordings, which is intended to enable for a quick overall examination of 
recorded interactions as well as for a more detailed inspection and comparison 
of multiple recordings.
Furthermore, it also provides an interface allowing other applications to make 
use of the recorded interactions and event data, e.g., for recommending tools.

We will make \mimesis open source so that other researchers can use it. 
\footnote{\url{https://www.anonymousurl.com/mimesis}}

% We intend to make \mimesis open source once it is a bit more matured 
% and has been tested more thoroughly in various recording scenarios so that 
% other researchers can use it.

% In the following sections, we will describe the recording and visualisation 
% features of \mimesis in more detail.

% \commentms{Einleitung Mimesis -- Eclipse plug-in, Visualisierung, wozu 
% überhaupt, nicht lang}
% 
% \commentms{aus Rainers email: "Wenn wir ankündigen, Mimesis open-source zu 
% machen, käme das vielleicht bei den Gutachtern auch gut an."}
% 
% \commentms{aus Rainers email: "zwei Hauptbeiträgen: (1) technische
% Infrastruktur für Entwicklerbeobachtungen durch Aufzeichnung von Interaktionen 
% in der IDE inklusive einer Visualisierung und (2) Beobachtungsstudie damit."}
% 
% \commentrk{Hier nochmal kurz eine Zusammenfassung der Ziele, die durch
%   die Aufzeichnung erreicht werden sollen. Generell sollte nach einer
%   Section noch etwas einleitender Text kommen, bevor die erste
%   Subsection beginnt. Was erwartet den Leser in dieser Section?}

\subsection{Recording Developer Behaviour}
\label{sec:recording}

% To record developers' behaviour, we implemented a plug-in for the 
% \textsc{Eclipse} IDE for Java, which is among the most popular IDEs for Java. 
When used in an \textsc{Eclipse} session, the \mimesis plug-in records almost 
every interaction that a developer performs with the IDE. 
Capturing as many interactions as possible is important, as every activity may 
indicate a certain state in the developer's task
completion~\citep{sillito2008asking, grigoreanu2012strategies, 
piorkowski2013whats, lawrance2013programmers}. 
% A good example for this is the consideration of alleged "idle times": if for 
If for a 
certain amount of time a developer does not perform an obvious action such as 
editing code, this could be considered to be an indication for the developer 
having left the desk, e.g., for going to the bathroom or fetching a cup of 
coffee~\citep{minelli2015know, amann2016study}.

On the other hand, it could also happen that the developer is just inspecting 
the code displayed on the screen very closely, maybe reading carefully.
% If only few events, e.g., just code-based edits are considered, a 
% differentiation between such cases is nearly impossible. 
% But if also rather subtle, not necessarily code-based interactions such as 
% general mouse movements are taken into account, this opens up a possibility to 
% reveal alleged "idle" phases to rather be times in which the developer is 
% passively working, e.g., by contemplating about what is currently displayed on 
% the screen.
% For instance, 
\citet{minelli2015know} noticed in their study on how developers 
spend their time programming, that there are at least two kinds of idle times: 
longer periods exceeding 5 minutes of duration, which they used to split 
% the interactions recorded by them into distinct development sessions and 
their recordings into distinct development sessions and
shorter idle times, which they \textit{explicitly} assumed to be periods of 
program understanding, e.g., time spent for reading and comprehending code.

\iffalse
For this reason, two special aspects were considered by us in particular, the 
one being to record all mouse actions, regardless if something was actually 
clicked or selected. 
This is done because some people tend to use the mouse on screen while reading 
in a way that one would use an index finger while reading a book, i.e., 
following the lines with the mouse pointer.
% \commentms{Ich meine, dass Amy Ko etwas zu diesen Eigenheiten von Entwicklern 
% geschrieben hatte. Nochmal nachschauen.}
Others would just keep their hand on the mouse, thus probably providing subtle 
movements that would allow to detect their presence.
The other aspect is to record the visible range, i.e., the first and last line 
of a text or code file that is currently visible on the screen, as users are 
not restricted in perceiving only the line that they are currently interacting 
with, but rather may read or perceive all visible surrounding lines as well, 
probably leading to the particular changes they are performing on the single 
line that they are actively interacting with.
Just evaluating code changes or similar active interactions may not be 
sufficient to comprehend developers' intentions nor provide insights into their 
current working state, as the \textit{code changes can be considered being 
just an effect of a cause} that is probably induced by rather 
"passive" interactions, 
i.e., by reading surrounding code. 
Those causes are to be recorded, albeit probably only possible indirectly, 
such as recording scrolling events, to provide a deeper and more 
complete insight into a developer's comprehension behaviour.
\fi

The individually recorded events are assigned to particular event categories, 
which are inspired by the work of \citet{proksch2018enriched} 
and \citet{minelli2014visualizing}.
Using such event categories allows for easier selection, search or filtering 
of event groups, e.g., filtering for code changing events only or selection of 
just navigation interaction for display in the visualisation.
The events currently recorded by the \mimesis plug-in include the following:
  
\begin{itemize}
\item \textsc{Activity}: \textit{a category for general activities, i.e., 
actions that do not correlate directly to a development 
activity}%\vspace*{\smallskipamount}
    \begin{itemize}
    \item RecordingEvent -- \textit{a recording starts / stops}
    \item ScrollEvent -- \textit{user scrolls inside an editor window}
    % (not in Navigation group, because it only changes the FOV of the 
% developer, not the cursor position
    \item TextSelectionEvent -- \textit {text is selected}
    \end{itemize} %\vspace*{\medskipamount}
    
\item \textsc{Execution}: \textit{events that involve running the 
program}%\vspace*{\smallskipamount}
    \begin{itemize}
    \item DebugEvent -- \textit{debugging related event, e.g., a breakpoint is 
set or hit}
    \item LaunchEvent -- \textit{project is executed or debugged}
    \item WebBrowserEvent -- \textit{the internal browser is launched, visited 
URLs and search queries are recorded}
    \end{itemize} %\vspace*{\medskipamount}
    
\item \textsc{Edit}: \textit{events relating to source code changes and 
annotations} %\vspace*{\smallskipamount}
    \begin{itemize}
    \item CodeChangeEvent -- \textit{source code in the IDE has been changed}
    \item CodeCompletionEvent -- \textit{code completion was used}
    \item TextCommentEvent -- \textit{developer added a textual comment 
        (within the \mimesis plug-in)}
    \item VoiceCommentEvent -- \textit{an audio comment has been added 
        (a special feature within the \mimesis plug-in)}
    \end{itemize} %\vspace*{\medskipamount}
    
  \item \textsc{Environment}: \textit{events that alter the IDE's 
appearance, such as changes to the IDE's main window, to a specific code editor 
window or changes to the IDE's views (representations of a project's metadata, 
such as properties or the project's file structure) or perspective (an initial 
collection and arrangement of views and an editor area)} 
%\vspace*{\smallskipamount}
    \begin{itemize}
    \item EditorEvent -- \textit{events specific to an editor window, e.g., 
resize or move}
    % \commentfg{Nur abstrakte Oberklasse zur internen Kategorisierung}
    \item PerspectiveEvent -- \textit{perspective is changed/opened}
    \item ViewEvent -- \textit{a view is opened/closed, or focus has changed 
within the IDE}
    \item WindowEvent - \textit{window focus of the IDE has changed, e.g., 
a different window was selected}
    \end{itemize} %\vspace*{\medskipamount}
    
\item \textsc{Navigation}: \textit{events related to developer navigation}
    \begin{itemize} %\vspace*{\smallskipamount}
    \item EditorMouseEvent -- \textit{mouse actions, such as clicking or moving 
the mouse} \vspace*{\smallskipamount}
    \item EditorTextCursorEvent -- \textit{text cursor was moved}
    \item SearchEvent -- \textit{a search query has been conducted}
    \item TreeSelectionEvent -- \textit{an element in the tree view was 
selected}
    \item TreeViewerEvent -- \textit{elements in the navigation view 
are collapsed/expanded}
    \end{itemize} %\vspace*{\medskipamount}
    
\item \textsc{Solution}: \textit{events related to solutions, the Eclipse 
name for application projects} %\vspace*{\smallskipamount}
    \begin{itemize}
    \item FileEvent -- \textit{event related to a single file}
%         \commentfg{Nur abstrakte Oberklasse zur internen Kategorisierung}
    \item ProjectEvent -- \textit{project has been loaded or unloaded}
    \item ResourceEvent -- \textit{files are created, deleted or changed}
    \item SaveEvent -- \textit{a file is saved}
    \end{itemize}
\end{itemize}

Beyond that, deviating from \citet{proksch2018enriched} 
and \citet{minelli2014visualizing}, for every event a reference to a special 
\texttt{EventContext} object is stored, which contains information about the 
corresponding event's environment, e.g., first and last line of code visible 
at the time the event took place. 
Furthermore, information about visible windows and tabs at the time 
of an event 
% of an interaction event 
is also stored in the context object.
% Furthermore, each recording stores a DisplayInformation object, which holds 
% information about the display environment, e.g., number of screens used and 
% resolution for each screen, which is meant to allow for better comparison 
% between recordings from different working environments. 

As the implementation of the event capturing is based on the \textsc{Eclipse} 
event bus system 
\footnote{\url{https://wiki.eclipse.org/Eclipse4/RCP/Event_Model}}, which 
is transporting events for virtually any interaction performed and event 
raised, also within the IDE, at nearly arbitrary granularity, from function 
calls to individual commands executed or buttons clicked, the addition of new 
events or event sources such as plug-ins to the IDE can be implemented using our 
event recording framework, which implements a wrapper around the Eclipse event 
bus, thus allowing for a straightforward extension, if needed.

\begin{figure*}[!htb]
  \centering
  \includegraphics[width=.8\textwidth]
  {img/imgUniF/ANBE_recording_2020-01-14-14-01-05_e} % \\[\bigskipamount]
  % \includegraphics[width=\textwidth]{img/legend2}
  \caption{Detailed visualisation of a developer's recorded interactions.}
  \vspace*{\smallskipamount}
  \textit{\footnotesize The graph displays the developer's navigation within 
the four files used, horizontal lines correspond to the visible range. 
Different symbols on the edges correspond to different types of performed 
interactions. Five code locations to be edited by the developer have been 
highlighted.}
  \label{fig:visualisation}
  \vspace*{-15pt}
\end{figure*}

\subsection{Visualising Developer Behaviour}

To further analyse recorded interactions, recorded data is transferred into a 
visual representation.
In contrast to existing, more abstract developer interaction visualisation 
approaches, ~\citep{grigoreanu2012strategies, minelli2014visualizing, 
piorkowski2013whats} we decided to use a graph-like visualisation using a kind 
of a "spatial" code representation, that would allow us to actually "see" the 
developer traverse between source code, documentation and other information. 
Within this visualisation the recorded developer navigation, e.g., line number 
location of interactions within corresponding files is plotted on the x-axis, 
while the y-axis was chosen to represent the chronological sequence of the 
recorded data (cf.~Figure~\ref{fig:visualisation}), bearing some similarity to 
how "tracks" are visually presented within video editing or similar composition 
software.
% Global Index
To enable the visualisation of interactions with multiple files, the index of 
the x-axis was chosen to be a concatenation of all lines contained in all files 
that the developer interacted with, i.e., the range of this "global index" 
is one to the sum of all lines contained in all files used by the developer, 
starting at the first line of the first file and advancing to the last line 
in the last file, using the number of lines in preceding files as an offset for 
subsequent files.
%Using this approach, which allows to represent source code files the way they 
%are actually structured, i.e., using their lines for x axis, our 
This representation 
enables researchers to observe the developer roaming through the code (and 
other files or 
documentation), using just a single graph.
As the computation of the global index is carried out based on specific rules, 
% \commentrk{Wirklich e.g. oder nicht eher i.e.? Oder kann man die 
% Reihenfolge aussuchen?}, 
e.g., alphabetical order of used files, directory structure or manually fixed 
order, this also allows for direct %side-by-side 
comparison of multiple 
recordings%(cf.~Figure~\ref{fig:multipleVisualisations}).
, e.g., between different developers.
%, which was one of the main objectives 
%of the 
% visualisation. 
To cope with the issue of emerging offsets and possible misalignment due to 
line additions and removals, we implemented an approach that maps such code 
in a way (we dubbed "code pockets") which maintains the original line number 
structure. % , this allowing for  
This approach also provides a code line mapping mechanism that allows for 
direct comparison of different recordings even if the file size was changed, 
e.g., one developer added or removed some lines of code to a file whereas 
another only edited existing lines of code.
% This is of special importance to us, as we plan to eventually compare multiple 
% interaction recordings on top of each other in a single visualisation, instead 
% of currently having to compare them side by side.

% % ROIs
% Another use of this deliberately chosen structure is the application of regions 
% of interest (ROI): As every recording visualisation (of the same task / source 
% code) can share the same structure for different developers by using a 
% respective definition of the global index, a mask to highlight areas of 
% particular importance, e.g., specific lines of code which would have to be 
% edited to complete a given task can be defined and applied to all 
% visualisations, thus allowing for a quick review, e.g., if a particular region 
% was visited / edited by a developer (cf.~Figure~\ref{fig:visualisation}).

% \commentms{display example ?}

% Tooltip and Event List
The visualisation itself most prominently displays the developer's navigation 
behaviour and viewing ranges, while also indicating particular interaction 
events by displaying corresponding point markers.
\iffalse
While a very great number for some events may occur in very quick 
succession and / or close space, thus leading to event data points covered by 
others, several mechanisms tackle this possible issue. 
To any point in the visualisation a contextual overlay is available which 
displays a list of all events below or near the current mouse position within 
the visualisation, additionally, a list of all recorded events is available at 
the edge of the visualisation. 
Clicking on any event data point in the visualisation makes the detailed event 
list jump to the corresponding event, a click on an event in the list makes the 
visualisation focus on that event.
\fi
To improve readability of the captured events, aggregation options are 
available, e.g., allowing to group subsequent keystroke events of a code change 
to a single event containing "before" and "after" states of the corresponding 
line, also allowing for escaping mechanisms, e.g., not grouping all subsequent 
keystrokes if there was a deletion in between, enabling 
comprehensibility of editing situations in which the developer changed his mind 
while typing.
Additionally, specific event types can be filtered and the edges of consecutive 
events can be individually enabled or disabled, allowing for 
individual visualisation scenarios such as only displaying events respresenting 
interactions that performed actual changes to the corresponding source code or 
only displaying navigation interactions while omitting code changes, for 
instance.
Furthermore, a level-of-detail (LOD) zooming feature allows to focus on a 
particularly interesting region or sequence of events displaying all events 
contained in that region with maximum detail, or to zoom out and reduce the 
number of events displayed while still maintaining the original shape of an 
interaction track for a broader overview of the complete recording. 
This feature is also significantly increasing the visualisation's performance 
and allows for inspection of very large recordings.
% In contrast to existing, more abstract developer interaction visualisation 
% approaches, ~\citep{grigoreanu2012strategies, minelli2014visualizing, 
% piorkowski2013whats} we decided to use a graph like visualisation using a kind 
% of a "spatial" code representation, that would allow us to actually "see" the 
% developer traverse between source code, documentation and other information. 
% Specifically, using our "global index" concept, which allows to represent 
% source code files the way they are actually structured, i.e., using their lines 
% for x axis, our representation enables to actually "see" the developer roaming 
% through the code.
\iffalse
Additionally, by representing every event recorded with individual 
datapoints that can be filtered for specific events or event categories our 
visualisation allows for a range of different visualisation scenarios: 
for a general overview, all events can be displayed at once, while for a more 
specific and detailed observation, individual events or event categories can be 
selected for display while others can be hidden, thus allowing for 
investigation of, e.g., only navigation behaviour or only editing behaviour, 
respectively.
To further enhance the comprehensibilty of a visualisation, the edges 
connecting consecutive events 
% which are used to illustrate the chronological sequence of events 
can be individually enabled or disabled for specific events 
or event categories, this allowing to highlight, e.g., tracks between 
navigation events or tracks between code changes, respectively. 
\fi

% \pagebreak
Alltogether, in contrast to other visualisation approaches, our approach is 
more 
fine-tuned to interactive utilisation, i.e., allows for many features such as 
selection and filtering of events and event categories and adjusting display 
properties to be configured interactively and overall aims more at the 
interactive investigation and comparison of a large number of recordings at 
once. %, than to represent single recordings.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mimesis_icpc2020"
%%% End:


==> references.tex <==
\section{Literature}

\begin{itemize}

    \item \citet{minelli2014visualizing} visualisation of developer 
        interactions with the Pharo IDE, stair diagram for developer 
        interactions, finds some action patterns, e.g., "inspection valley"

    \item \citet{baltes2015navigate} matching appropriate information display 
        and working steps, negative influence of "split-attention" effect

    \item \citet{bazrafshan2014effect} developers neglecting useful information
    
    \item \citet{furnas1987vocabulary} wrong expectations due to function names
    
    \item \citet{grigoreanu2012strategies} assumptions about program 
        comprehension work steps, differentiated different work steps, i.e., 
        "schema step"
    
    \item \citet{guzzi2011bookmarks} developers did not make use of a specific 
        tool for program comprehension in active development, in spite of the 
        tool in question being congruently reported to be useful and easy to 
        use by the developers in question.

    \item \citet{ko2007information} observation study (n=17, n'=49), "explain 
        to newcomer" self-reporting scenario, identification of 21 types 
        of information sought by programmers in software development

    \item \citet{ko2006exploratory} Observation study (n=10, n'=31), developers 
        had to fix 5 "issues" (individual tasks) in a program (java swing, 
        medium size, spread across 9 classes and 9 files) using the Eclipse 
        IDE. The observed developers displayed different strategies and 
        differed in what code segments they considered to be of importance (for 
        the respective task to be solved).

    \item \citet{ko2003individual} observation study (n=75), video transcript 
        recording of behavior, different tasks, not only computer experts, but 
        also experts from other domains (psychology), good statistical 
        coverage, cluster analysis; Ss displayed 3 distinct comprehension 
        strategies: depth-first (below average programming experience Ss), 
        breadth-first (high programming experience Ss) and "passive" (least 
        programming experience Ss) comprehension strategy

    \item \citet{lawrance2008using} application of information foraging theory
    
    \item \citet{lawrance2013programmers} observation of developers' behaviour 
        according to information foraging theory, differentiation of bug fixing 
        tasks (e.g., "missing feature" and "broken feature"), working steps 
        analysis, effectiveness of information scents
        
    \item \citet{maalej2014comprehension} Respondents of a questionnaire 
        reported different information needs corresponding to the task they 
        would have to solve. "Wherever possible, developers seem to prefer 
        strategies that avoid comprehension, because of time and mental effort 
        needed. Program comprehension is rather considered as a necessary step 
        to accomplish different maintenance tasks rather than a goal by 
        itself." "One of our most interesting findings is that developers put 
        themselves in the role of users at the start of a comprehension process 
        and try to collect and comprehend usage data. (...) This strategy aims 
        at understanding the program behavior and structure and at getting 
        first hints for further program exploration – an alternative to reading 
        and debugging source code." "Our results reveal a gap between research 
        and practice as we did not observe any use of comprehension tools and 
        developers seem to be unaware of them. Overall, our findings call for 
        reconsidering the research agendas towards a context-aware tool 
        support."
    
    \item \citet{oliveira2014security} offers explanation of bad / negligent 
        software development (in respect of security aspects) by the assumption 
        that developers stick to heuristic-based decision-making processes, 
        security is not part of the heuristics used by developers in their 
        daily programming tasks
    
    \item \citet{pirolli2007information} Information Foraging Theory
    
    \item \citet{pirolli1999information} application of the Optimal Foraging 
        Theory to human information understanding - when searching for 
        information, humans ("Informavores") use "built-in" foraging 
        mechanisms, essentially trying to maximize information gain while 
        minimizing searching effort. "Information scents" indicate the chances 
        to find useful information on a search path,
    
    \item \citet{roehm2012professional} "Wissen, das geteilt wird, entspricht 
        nicht den ben\"otigten Informationen", "Verwendung [von Tools zum 
        Programmverstehen] bedeutet unattraktiven Mehraufwand", Entwickler 
        zeigten unterschiedliche Strategien zur Bew\"altigung von 
        Programmieraufgaben, w\"ahlten jedoch in Abh\"angigkeit vom jeweiligen 
        Aufgabenkontext eine von ihnen als geeignet erscheinende Strategie
    
    \item \citet{rugaber1995program} definition of the term "program 
        comprehension"
    
    \item \citet{sadowski2015developers} "almost a third of searches are 
        incrementally performed through query reformulation" --> recursive 
        search
    
    \item \citet{sillito2008asking} Observations and qualitative studies to 
        understand associated activities of programmers performing a change 
        task. Four categories of questions asked by programmers, expressing a 
        hierarchy of steps for program comprehension: a) finding focus points, 
        b) expanding focus points, c) understanding a subgraph and d) questions 
        over groups of subgraphs
    
\end{itemize}

